Uncovering Temporal Context for Video Question and Answering

In this work, we introduce Video Question Answering in temporal domain to infer the past, describe the present and predict the future. We present an encoder-decoder approach using Recurrent Neural Networks to learn temporal structures of videos and introduce a dual-channel ranking loss to answer multiple-choice questions. We explore approaches for finer understanding of video content using question form of "fill-in-the-blank", and managed to collect 109,895 video clips with duration over 1,000 hours from TACoS, MPII-MD, MEDTest 14 datasets, while the corresponding 390,744 questions are generated from annotations. Extensive experiments demonstrate that our approach significantly outperforms the compared baselines.

==> back.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|c|}
               & TACoS  & MPII-MD & MED \\
\hline\hline
               &        &         & \\
    $\lambda_0=0.1$ &        &         &\\
            &        &         &\\
\hline
               &        &         & \\
    $\lambda_0=0.3$ &        &         &\\
            &        &         &\\
\hline
               &        &         & \\
    $\lambda_0=0.5$ &        &         &\\
            &        &         &\\
\hline
               &        &         & \\
    $\lambda_0=0.7$ &        &         &\\
            &        &         &\\
\hline
               &        &         & \\
    $\lambda_0=0.9$ &        &         &\\
            &        &         &\\
\end{tabular}
\end{center}
\caption{Comparison of diffrent $\lambda_0$}
\end{table}

%\begin{figure}
%\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %%\includegraphics[width=0.8\linewidth]{egfigure.eps}
%\end{center}
   %\caption{Effectiveness of multi-layer transformation layer}
%\label{effectiveness_of_multilayer_transformation_layer}
%\end{figure}

\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|c|}
               & TACoS  & MPII-MD & MED \\
\hline\hline
               &        &         & \\
    $\lambda_0=0.1$ &        &         &\\
            &        &         &\\
\hline
               &        &         & \\
    $\lambda_0=0.3$ &        &         &\\
            &        &         &\\
\end{tabular}
\end{center}
\caption{Comparison between different types of questions}
\end{table}


==> expr_bak.tex <==
%\subsection{Baselines and training detail}

%\textbf{Baselines} To evaluate our proposed model, we designed the following baselines for comparison.
%One simplest baseline is to randomly pick an answer from candidates. For easy task, the performance would
%be about 25\% and 10\% for hard task.
%We evaluate the performance with randomly initialization the transformation layers.
%We will compare our model with a set of stronger baselines.
\begin{comment}
\begin{enumerate}
    \item \textbf{CCA}
      Canonical Correlation Analysis (CCA) \cite{hotelling1936relations} computes the directions of maximal correlation between a pair of multi-dimensional variables.
      We perform linear CCA for visual and sentence embedding, as well as visual and phrase embedding.
      As to answer questions, we embed each candidates and calculate the score of Equation \ref{score_equation}.
      We grid search the best $\lambda_0$ based on validation set.
    %\item \textbf{BLIND}
          %Another baseline would be eliminate visual information and answer questions only based on the semantic features.
          %We use the following score
            %\begin{equation}
                %score = \lambda_0I^TW_{sv}S_{ij} + (1-\lambda_0)I^TW_{pv}P_{ij}
                %\label{score_equation_text_only}
            %\end{equation}
          %where $I$ is a all one vector. The idea behind this score is that we treat the visual information for each question to be identical,
          %which in another way discards the visual part. The corresponding loss function is the same as Equation \ref{loss_function_equation},
          %where visual embeddings constant.
    \item \textbf{Sentences only and phrases only}
          In this model, we also train embedding only with sentences or phrases.
          Note that it is a special case of Equation \ref{score_equation} where $\lambda_0$ is $1$ or $0$.
          By comparing with this method, we can demonstrate whether combining sentence description and phrases will help improve the performance.
     \item \textbf{Visual with avg CNN}
    \label{visual_avg_cnn}
           %All previous baselines use our encoder model to learn visual features.
           We also evaluate the effectiveness of our visual encoder-decoder model by comparing with directly average CNN features.
           We use the same underlying CNN model as encoder-decoder model. Thus we just replace the visual feature with CNN feature.
           The comparison is reasonable as both feature are with same dimension of 1024 and we use the same transformation layer as well.
           %When it comes to the task of describing the past and future, we simply use the visual feature from the current clip.
           %We add the past and future experiment as it is interesting to see what would the model behave when the visual and semantic information are inconsistent.
    %\item \textbf{Visual with GRU encoder}
          %In our proposed full model, we furthermore evaluate the past and future model by comparing the performance
          %with directly using the present model just like in Baseline \ref{VISUAL_AVG_CNN}
          %where we use the current clip representation for past and future modeling.
\end{enumerate}

\textbf{Comparison with CCA}.
\label{compare_with_cca}
We perform comparison between CCA and our ranking loss algorithm. For visual input feature,
we average features extracted from GoogLeNet for each frame.
For semantic features, we use skip-thought vector to encode sentences and word2vec to encode
phrases (averaging each word representation).
We fix $\alpha$ and $\beta$ to 0.2 and 0.1 for both case, and $\lambda_0$ is cross-validated.
For CCA, instead of sampling examples from training data, we use all instances to in
the training set to learn a joint embedding. We learn two separate embedding,
visual feature of 1024 dimension and sentence of 4800, visual feature of 1024 dimension and phrase of 300.
As for our ranking loss, we train with stochastic gradient descent and set the learning rate to 0.01, momentum to 0.9.
Dimension of visual sentence embedding is set to 500 and 300 for visual phrase embedding.
Results are shown in Table \ref{cca_campare}.
We can see that our simple ranking loss outperform
the CCA by a large margin in three datasets.

\textbf{Analysis of sentence and phrase weight}
\label{sentence_and_phrase_weight}
We show the effectiveness of combining sentence and phrase during learning process.
We experiment on present easy task. The result is shown on Figure \ref{global_and_local_comp}.
As we can see that combining sentence and phrase does improve the performance.

\textbf{Comparison between GRU encoder and averaging of CNN features}
We show that GRU encoder improve the performance by comparing with a strong baseline of
averaging CNN features for each frame.

\input{./table/expr/cca_table.tex}
\input{./table/expr/gru_cnn_comp_table.tex}
\input{./table/expr/gru_all_table.tex}

\begin{figure}
\begin{center}
    \includegraphics[height=0.2\linewidth]{./images/global_and_local.png}
\end{center}
   \caption{Comparison of different $\lambda_0$}
\label{global_and_local_comp}
\end{figure}

\begin{figure}
\begin{center}
    \includegraphics[width=1.0\linewidth]{./images/Showing_case_of_result.png}
\end{center}
   \caption{Comparison of different $\lambda_0$}
\label{global_and_local_comp}
\end{figure}

\begin{figure*}
\begin{center}
   \includegraphics[width=1.0\linewidth]{./images/show_overall_result.png}
\end{center}
   \caption{Example result of our proposed}
\label{full_model_result}
\end{figure*}

\subsection{Results and analysis}
We visualize part of the experiment results of our full model in Figure \ref{full_model_result}.

\textbf{The effectiveness of past and future model}

\textbf{The effectiveness of combing sentence and phrase features}

\textbf{Comparison between answering different types of questions}
\subsection{Limitations}
\end{comment}


==> table/expr/cate_result_table.tex <==
\begin{table}
\footnotesize
\begin{center}
\begin{tabular}{lc|c|c|c}
Dataset &   & Actions & Objects & Phrases \\
\hline\hline
& Past &  &    & \\
TACoS & Future &   &   & \\
      & Present &  &    & \\
\hline
        & Past   &   &   \\
MPII-MD & Present  &   &   \\
        & Future  &   &   \\
\hline
      & Past &      &\\
MEDTEST14 & Present &      & \\
      & Future &      & \\
\hline
\end{tabular}
\end{center}
\caption{Result for each category}
\label{cate_result_table}
\end{table}


==> table/expr/cca_vs_our_table.tex <==
\begin{table}
\footnotesize
\begin{center}
\begin{tabular}{lc|c|c}
    Datasets & Splits & CCA & Our model \\
\hline\hline
          & split 1 &  66.2\%  & 65.5 \% \\
TACoS     & split 2 &  64.0\%  & 66.0 \% \\
          & split 3 &  66.3\%  & 68.1 \% \\
          & mean    &  65.5\%  & 66.5 \% \\
\hline
          & split 1 &  45.8\%  & 45.2 \% \\
MPII-MD   & split 2 &  49.8\%  & 50.2 \% \\
          & split 3 &  46.3\%  & 46.8 \% \\
          & mean    &  47.3\%  & 48.1 \% \\
\hline
           & split 1 & 60.9\%  & 61.4 \% \\
MEDTEST 14 & split 2 & 60.9\%  & 61.1 \% \\
           & split 3 & 60.4\%  & 62.3 \% \\
           & mean    & 60.7\%  & 61.6 \% \\
\hline
\end{tabular}
\end{center}
\caption{Comparison between ConvNets average and our model on \textit{Present-Hard} task.}
\label{gru_cnn_comp_table}
\end{table}


==> table/expr/gru_cnn_comp_table.tex <==
\begin{table}
\footnotesize
\begin{center}
\begin{tabular}{lc|c|c}
    Datasets & Splits & ConvNets Average & Our model \\
\hline\hline
          & split 1 &  66.2\%  & 65.5 \% \\
TACoS     & split 2 &  64.0\%  & 66.0 \% \\
          & split 3 &  66.3\%  & 68.1 \% \\
          & mean    &  65.5\%  & 66.5 \% \\
\hline
          & split 1 &  45.8\%  & 45.2 \% \\
MPII-MD   & split 2 &  49.8\%  & 50.2 \% \\
          & split 3 &  46.3\%  & 46.8 \% \\
          & mean    &  47.3\%  & 48.1 \% \\
\hline
           & split 1 & 60.9\%  & 61.4 \% \\
MEDTEST 14 & split 2 & 60.9\%  & 61.1 \% \\
           & split 3 & 60.4\%  & 62.3 \% \\
           & mean    & 60.7\%  & 61.6 \% \\
\hline
\end{tabular}
\end{center}
\caption{Comparison between ConvNets average and our model on \textit{Present-Hard} task.}
\label{gru_cnn_comp_table}
\end{table}

